Observability and Identifiability Analyses of Process Models for Agricultural Anaerobic Digestion Plants

Dynamic operation of anaerobic digestion plants requires advanced process monitoring and control. Different simplifications of the Anaerobic Digestion Model No. 1 (ADM1) have been proposed recently, which appear promising for model-based process automation and state estimation. As a fundamental requirement, observability and identifiability of these models are analyzed in this work, which was pursued through algebraic and geometric analysis. Manual algebraic assessment was successfull for small models such as the ADM1-R4 and simplified versions of the ADM1-R3, which were derived in this context. However, for larger model classes the algebraic approach showed to be insufficient. By contrast, the geometric approach, implemented in the STRIKE_GOLDD toolbox, allowed to show observability for more complex models (including ADM1-R4 and ADM1-R3), employing two independent algorithms. The present study lays the groundwork for state observer design, parameter estimation and advanced control resting upon ADM1-based models.

==> Input/Results.tex <==
\section{Results and Discussion}
% 
\subsection{Algebraic Approach}
\label{sec:res:algApproach}
%
The full ADM1-R4 (BMR4+AB) could be shown to be globally observable by using the measurements %(and their time derivatives) 
given in Tab.~\ref{tab:res:algApproach}. The underlying system of equations involves online measurements of the gas composition (CH\textsubscript{4} and CO\textsubscript{2}). %(partial pressures of CH4 and CO2) 
%and their first and second time derivatives. Furthermore, 
%offline measurement values (without time derivative) 
Furthermore, to guarantee observability, measurements of IN, TS and VS need to be available. This follows directly from the model equations: all three states only appear in their corresponding differential equation. % XY: see SI 
Therefore, if they were not available as measurements, they could not be observable because they would not be introduced into the system of equations via other measurements, regardless of the degree of time derivatives. 
%
\begin{table}[t]
	\scriptsize
	\vspace*{-7pt}
	\renewcommand{\arraystretch}{1.5}
	\caption{Measurements and their time derivatives required for algebraic observability of model simplifications}
	\label{tab:res:algApproach}
	\centering
	\setlength\tabcolsep{3pt}
	\begin{tabular}{|l|r|r V{3} *{5}{c|}c V{3} *{3}{c|}c V{3} *{3}{c|}c V{3} c|c|}
		\hline
		\multicolumn{3}{|l V{3}}{} & \multicolumn{6}{c V{3}}{\textbf{Nominal measurements}$^{\mathrm{a,b}}$} & \multicolumn{4}{c V{3}}{\textbf{1\textsuperscript{st} derivative}} & \multicolumn{4}{c V{3}}{\textbf{2\textsuperscript{nd} derivative}} & \multicolumn{2}{c|}{\textbf{3\textsuperscript{rd} deriv.$^{\mathrm{e}}$}} \\
		\hline
		\textbf{Model name} & $n^{\mathrm{c}}$ & $t [s]^{\mathrm{d}}$ & CH\textsubscript{4} & CO\textsubscript{2} & IN & TS & VS & Ac & CH\textsubscript{4} & CO\textsubscript{2} & IN & TS & CH\textsubscript{4} & CO\textsubscript{2} & IN & TS & CH\textsubscript{4} & CO\textsubscript{2} \\
		%
		\hline
		BMR4 	& 9 & 5 	& x & x & x & x & x & 	& x & x & & & x & x & & & & \\
		\hline
		BMR4+A 	& 9 & 3 	& x & x & x & x & x & 	& x & x & & & x & x & & & & \\
		\hline
		BMR4+B 	&11 & 6 	& x & x & x & x & x & 	& x & x & & & x & x & & & x & x \\
		\hline
		BMR4+AB &11 & 8 	& x & x & x & x & x & 	& x & x & & & x & x & & & x & x \\
		\specialrule{.12em}{0.01em}{0.01em} 
		\multirow{2}*{BMR3+AC}$^{\mathrm{f}}$ &\multirow{2}*{11} & 1092& x & x & x & x & x & x & x & & x & x & x & & x & & & \\
		& & 1065& x & x & x & x & x & x & x & & x & x & x & & & x & & \\
		\hline
		\multirow{2}*{BMR3+BC}$^{\mathrm{f}}$ & \multirow{2}*{13} & 5352 & x & x & x & x & x & x & x & x & x & x & x & x & x & & & \\
		& & 6353 & x & x & x & x & x & x & x & x & x & x & x & x & & x & & \\
		\hline
		\multirow{2}*{BMR3+ABC}$^{\mathrm{f}}$&\multirow{2}*{13} & 3861	& x & x & x & x & x & x & x & x	& x & & x & x & & & x & x \\
		&	& 8730 & x & x & x & x & x & x & x & x	& & x & x & x & & & x & x \\
		%& & & & & & & & & & & & & & & & & & \\ % leere Zeile
		\hline
		\multicolumn{19}{l}{$^{\mathrm{a}}$CH\textsubscript{4}, CO\textsubscript{2} - partial pressures of methane and carbon dioxide; IN - inorganic nitrogen; TS, VS - total and volatile} \\
		\multicolumn{19}{l}{solids; Ac - acetic acid \quad $^{\mathrm{b}}$CH\textsubscript{4} and CO\textsubscript{2} were assumed as online measurements, as well as Ac for ADM1-R3 } \\
		\multicolumn{19}{l}{variants. IN, TS and VS were assumed as offline measurements. \quad $^{\mathrm{c}}$Number of states \quad $^{\mathrm{d}}$Computation time}\\
		\multicolumn{19}{l}{$^{\mathrm{e}}$derivative \quad $^{\mathrm{f}}$Only local observability could be shown because two solutions to the equation systems were found.}
		%\multicolumn{19}{l}{}
	\end{tabular}
\end{table}
%

Model simplifications were applied to the ADM1-R4, resulting in the submodels BMR4, BMR4+A and BMR4+B. This was done to explore the effect of individual model parts on the complexity of the system of equations, indicated by the computation time required to solve the system of equations. 
%This had two reasons: first, to draw a complete picture of the analysis; and second, to learn about the effect individual model parts have on the complexity of the equation system, indicated by the computation time required to solve the equation system. 
However, reduction in computational complexity could not clearly be attributed to omitted model parts, as summarized in Tab.~\ref{tab:res:algApproach}: The simplest model variant (BMR4) showed the second highest computation time among the ADM1-R4 models, whereas the fastest computation time could be achieved with the less reduced variant BMR4+A. Nevertheless, all \mbox{ADM1-R4} submodels could be shown to be globally observable and required only short computation times. 

For the full ADM1-R3 (BMR3+ABCDE), the solver of Mathematica failed to deliver conclusive statements on observability, likely due to the complexity of the resulting 
%symbolic
terms in the system of equations. Neither a set of solutions nor an empty set could be returned. Instead, the kernel systematically died in the process of solving the system of equations. Hence, with the algebraic approach, observability of the full ADM1-R3 could not be determined. Therefore, model complexity of the ADM1-R3 was reduced by isolating and omitting individual model parts (see Sec.~\ref{sec:meth:ADModels}). 

%Observability of individual ADM1-R3 submodels is described in the following, progressing from simple to more complex models. 
Up to this point, measurements of CH\textsubscript{4}, CO\textsubscript{2}, IN, TS and VS were assumed. Additionally, for all ADM1-R3 submodels online measurements of acetic acid had to be taken into account to show local observability, see Tab.~\ref{tab:res:algApproach}. The obtained results are therefore strictly valid only for lab- and pilot-scale settings \citep{Boe.2012}. 
%(\textbf{XY:} hier evtl. noch Kagen (TU Wien) zitieren, die Modelle erst durch Hinzunahme weiterer Messungen beobachtbar macht.) 
%Global observability could be shown for the model variants BMR3+ABC and BMR3+AC, and local observability for BMR3+BC.
To find solutions of the systems of equations, first and second-order derivatives of the offline measurements IN and TS are required, see Sec.~\ref{sec:meth:dataAvailability}. %, for which we assumed sample-and-hold behavior. 
%Except at the sampling points, these derivatives are assumed to be zero (sample-and-hold behavior, see Sec.~\ref{sec:meth:dataAvailability}). 

With given nominal values of VS, it was preferred to include time derivatives of TS over VS, because both terms added the same information to the system of equations but TS delivered less complex terms. 

For both BMR3+AC and BMR3+BC, local observability could be shown for two combinations of equations, each only differing by one equation: the second derivative of IN or of TS, as shown in Tab.~\ref{tab:res:algApproach}. Both respective combinations were solved in similar computation times. 

BMR3+ABC is the most complex model variant which still delivered a solution of the resulting system of equations. Two solutions of the systems of equations each could be found by either incorporating the first derivative of IN or TS. The latter resulted in more than double computation times (Tab.~\ref{tab:res:algApproach}). Based on specific model equations, this was not expected because the first derivatives of both IN and TS have the same algebraic structure and are linearly dependent except for their convection terms. % (\textbf{XY:} see SI). 

By contrast, for BMR3+AC and BMR3+BC computation times of the two respective solutions did not differ much. This indicates that computational complexity of the terms resulting from the second derivatives of IN and TS does not change as much as for their first derivatives (observed in BMR3+ABC). Omitting model part~B (cf. BMR3+AC) resulted in a significant reduction of computation times, which is in line with the findings for ADM1-R4 model variants. Omitting part~A instead does not allow to draw such clear conclusions  (cf. BMR3+BC), since computation times are in between the two observable combinations of BMR3+ABC. 

When restricting measurements %and their time derivatives
to gas composition, IN, TS and VS, none of the ADM1-R3 submodels could be shown to be observable using the algebraic approach. 
For higher-order variants than BMR3+ABC, inhibition through pH and ammonia need to be considered, as well as computation of pH. This entails a higher number of state variables, which leads to symbolic systems of equations too complex to be solved in the presented framework. 

Lower-order model variants of the ADM1-R3 were not considered because (i) no clear tendency of reduction in computation time could be observed by omitting model parts, and (ii) for practical applications, lower-order models were already given through the ADM1-R4 and corresponding submodels.
%
\subsection{Geometric Approach}
% 
Based on the implementation in the STRIKE\_GOLDD toolbox, the geometric approach proved to be successful in showing both local observability and structural local identifiability of the full models ADM1-R4 and ADM1-R3. Moreover, this was achieved in (i) considerably shorter computation times, (ii)~without assuming acetic acid as an online measurement, and (iii) by employing two independent algorithms (FISPO and ORC-DF). This is summarized in Tab.~\ref{tab:res:geomApproach}. %For comparison, the table also included BMR3+ABC, being the most complex model variant for which local observability could be shown under the algebraic approach. 
As noted by \citep{Martinez.2020}, computational efficiency of FISPO and ORC-DF can differ vastly depending on the model structure, which is apparent for the larger ADM1-R3. 

Furthermore, computational effort decreases significantly when neglecting model parts of the full ADM1-R3: computation times of the submodel BMR3-ABC, for instance, could be reduced to 12 and \SI{5}{\second} for the FISPO and ORC-DF algorithms, respectively. This is also considerably faster than those computation times achieved with the algebraic approach, cf. Tab.~\ref{tab:res:algApproach}.
%Note the massive difference in computation times.
%
\begin{table}[tb]
	\renewcommand{\arraystretch}{1.1}
	\caption{Model properties and computation times of FISPO and ORC-DF algorithms for ADM1-R4 and ADM1-R3.}%, and BMR3+ABC}
	\centering
		\begin{tabular}{|l|r|r|r|r|}
		\hline
		\multirow{2}{*}{\textbf{Model class}} & \multicolumn{2}{c|}{\textbf{number of}} & \multicolumn{2}{c|}{\textbf{computation time in s}} \\
		\cline{2-5} 
		 & \textbf{states} & \textbf{parameters} & \textbf{FISPO} & \textbf{ORC-DF} \\
		%
		\hline
		%
		ADM1-R4 & 11 & 4 & 3 & 7 \\
		\hline 
%		BMR3+ABC& 13 & 7 & 26 & 6 \\
%		\hline 
		ADM1-R3 & 17 & 7 & 11959 & 811 \\
		\hline
		%			\multicolumn{3}{l}{$^{\mathrm{a}}$} \\
		\end{tabular}
		\label{tab:res:geomApproach}
\end{table}
%

Higher-order model classes such as the ADM1-R2 are of similar structure as the ADM1-R3, but involve significantly more time-variant parameters and contain a more detailled acid spectrum (acetic to valeric acid instead of only acetic acid) \citep{Weinrich2021b}. In an agricultural setting, these acid measurements are not available online. However, even when assuming them to be available as online measurements, both algorithms of the geometric approach fail to deliver conclusive statements. This is likely due to the aggravated complexity of the involved symbolic expressions. 

A practical application of the ADM1-R2 is thus not anticipated for monitoring and control schemes due to the lack of online measurements for the individual VFA. It was therefore not further simplified into submodels and no further observability and identifiability analyses were pursued. 
%The presented results are only of theoretical nature. The full ADM1-R3 involves 17 states and 7 time-varying parameters, which all have to estimated from a scarce number of measurements in a practical setting. 

